Tighter Bounds on the Expressivity of Transformer Encoders

Characterizing neural networks in terms of better-understood formal systems has the potential to yield new insights into the power and limitations of these networks. Doing so for transformers remains an active area of research. Bhattamishra and others have shown that transformer encoders are at least as expressive as a certain kind of counter machine, while Merrill and Sabharwal have shown that fixed-precision transformer encoders recognize only languages in uniform $TC^0$. We connect and strengthen these results by identifying a variant of first-order logic with counting quantifiers that is simultaneously an upper bound for fixed-precision transformer encoders and a lower bound for transformer encoders. This brings us much closer than before to an exact characterization of the languages that transformer encoders recognize.

==> nn.tex <==
\RequirePackage{tikz}
\RequirePackage{pgfplots}
\tikzset{>=stealth}
\tikzset{every edge/.style={draw,auto=right,font={\tiny},inner sep=0.5mm,outer sep=0mm}}
\tikzset{bias/.style={label=right:{\tiny #1}}}
\tikzset{unit/.style={draw,circle,minimum size=4mm}}
\tikzset{input/.style={unit,node contents={}}}
\tikzset{linear/.style={unit,inner sep=0mm,node contents={%
\begin{tikzpicture}[x=2mm,y=2mm,baseline=0]
\draw (-0.6,-0.6) -- (0.6,0.6);
\end{tikzpicture}%
}}}
\tikzset{relu/.style={unit,inner sep=0mm,node contents={%
\begin{tikzpicture}[x=2mm,y=2mm,baseline=0]
\draw (-0.707,0) -- (0,0) -- (0.707,0.707);
\end{tikzpicture}%
}}}
\tikzset{sigmoid/.style={draw,circle,inner sep=0mm,minimum size=6mm,node contents={%
\begin{tikzpicture}[baseline=0]
\begin{axis}[width=20mm,height=20mm,axis x line=none,axis y line=none]
\addplot[mark=none] {1/(1+exp(-x))};
\end{axis}
\end{tikzpicture}%
}}}
\tikzset{att/.style={draw,rectangle,minimum width=1cm,minimum height=1cm,node contents={Att}}}
\tikzset{every label/.style={font={\small}}}

